Community Discovery in Dynamic Networks: a Survey

Networks built to model real world phenomena are characeterised by some properties that have attracted the attention of the scientific community: (i) they are organised according to community structure and (ii) their structure evolves with time. Many researchers have worked on methods that can efficiently unveil substructures in complex networks, giving birth to the field of community discovery. A novel and challenging problem started capturing researcher interest recently: the identification of evolving communities. To model the evolution of a system, dynamic networks can be used: nodes and edges are mutable and their presence, or absence, deeply impacts the community structure that composes them. The aim of this survey is to present the distinctive features and challenges of dynamic community discovery, and propose a classification of published approaches. As a "user manual", this work organizes state of art methodologies into a taxonomy, based on their rationale, and their specific instanciation. Given a desired definition of network dynamics, community characteristics and analytical needs, this survey will support researchers to identify the set of approaches that best fit their needs. The proposed classification could also help researchers to choose in which direction should future research be oriented.

==> living_survey.tex <==
One of the major drawbacks of research surveys is that they are subject to rapid aging.
Nowadays, the exponentially growing number of scientific publications puts a strain on researchers cognitive abilities: it is nearly impossible to keep track of all the works that are continuously published on specific topics.
Surveys are designed to capture (often partial) snapshots of the state of art, of specific fields, at a given time: for this reason, they cannot be used as up to date references.
Even though they are really useful to scholars that need to approach a specific topic for the first time, their lack of updated references make them useless as starting point for the identification of actual trends among the scientific community.
For this reason we decided to transform the present work in a \emph{Living Survey}.
In order to always maintain up to date the contents discussed in the current survey, we release a dedicated website\footnote{Living Survey url available at camera ready stage} whit the aim of keeping track of novel researches on Dynamic Community Discovery.
On the living survey website are made available information regarding dynamic community discovery approaches, datasets, evaluation methodologies and visual tools. 
We encourage authors to participate with information about their works (as well as other resources): all contributions will be categorized, linked and made available online.
Dynamic Community Discovery is a relatively novel topic that is likely to attract increasing attention in the future: our goal is to provide scholars with a complete reference of existing works and methodologies and to build a community around researchers that works in the dynamic network analysis field.
